Swift and SALT observations of the Multiple Outbursts of MAXI J1957+032

The new recurrent X-ray transient MAXI J1957+032 has had four X-ray outbursts within 16 months, all very briefly detected (lasting <5 days). During the most recent event (Sep/Oct 2016), we obtained with SALT the first optical spectrum of the transient counterpart, showing the classic blue continuum of an X-ray irradiated disc in an LMXB and no other features. At high Galactic latitude below the plane (-13 deg) reddening is low but there is no quiescent counterpart visible on any of the existing sky surveys, nor any other known X-ray source in the region. Swift monitoring of 3 of the 4 events is presented, showing rapidly fading X-ray outbursts together with significant UVOT detections in the UV (W1,M2,W2), U and B bands. The optical properties are most like those of the short-period LMXBs, which, combined with the softening witnessed during the decay to quiescence would place the system at d <13 kpc. The short duration and short recurrence time of the outbursts are reminiscent of the AMXPs, which exhibit peak luminosities of 1 % L_Edd. Assuming this peak luminosity would place MAXI J1957+032 at a distance of d= 5-6 kpc.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\apss{Ap\&SS}
\def\apjs{ApJS}
\def\araa{ARA\&A}
\def\pasp{PASP}
\def\aj{AJ}
\def\ssr{SSR}

==> definitions.tex <==
\newcommand{\he}[1] {He\,{\sc #1}}
\newcommand{\hel}[2] {He\,{\sc #1}~$\lambda$#2}
\newcommand{\ha}{H$\alpha$ }
\newcommand{\hb}{H$\beta$}
\newcommand{\hg}{H$\gamma$}
\newcommand{\hd}{H$\beta$}
\newcommand{\hep}{H$\epsilon$}
%\newcommand{\ionl}[3] {#1\,{\sc #2}~$\lambda$#3}
%\newcommand{\ion}[2] {#1\,{\sc #2}}


%\newcommand{\ca}[1] {\citealt{#1\}}
%
% de aapp4
%
\def\kms{\mbox{${\rm km}\:{\rm s}^{-1}\:$}}
\def\ms{${\rm m}\:{\rm s}^{-1}\:$}

\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\let\la=\lesssim
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\let\ga=\gtrsim
\def\fdg{\hbox{$.\!\!^\circ$}}
\newcommand{\fdeg}{\hbox{$.\!\!^\circ$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\kmm{${\rm km}^{-1}$}
\def\d{{\rm d}}
\def\degree{\mbox{$^{\circ}$}}
\def\sol{~\mathrm{M}_\odot}
\def\lx{$L_\mathrm{X}$}
\def\kem{$K_\mathrm{em}$}
\def\ergs{erg s$^{-1}$}
\def\ledd{$L_\mathrm{Edd}$}

%Sloan filters
\def\sloanu{$u^\prime$}
\def\sloang{$g^\prime$}
\def\sloanr{$r^\prime$}
\def\sloani{$i^\prime$}
\def\sloanz{$z^\prime$}

%Colours
\newcommand{\red}[1] {\textcolor{red}{#1}}
\newcommand{\redp}[1] {\textcolor{red}{(#1)}}	%entre parentesis
\newcommand{\blue}[1] {\textcolor{blue}{#1}}
\newcommand{\green}[1] {\textcolor{green}{#1}}

